Associating Spatially-Consistent Grouping with Text-supervised Semantic Segmentation

In this work, we investigate performing semantic segmentation solely through the training on image-sentence pairs. Due to the lack of dense annotations, existing text-supervised methods can only learn to group an image into semantic regions via pixel-insensitive feedback. As a result, their grouped results are coarse and often contain small spurious regions, limiting the upper-bound performance of segmentation. On the other hand, we observe that grouped results from self-supervised models are more semantically consistent and break the bottleneck of existing methods. Motivated by this, we introduce associate self-supervised spatially-consistent grouping with text-supervised semantic segmentation. Considering the part-like grouped results, we further adapt a text-supervised model from image-level to region-level recognition with two core designs. First, we encourage fine-grained alignment with a one-way noun-to-region contrastive loss, which reduces the mismatched noun-region pairs. Second, we adopt a contextually aware masking strategy to enable simultaneous recognition of all grouped regions. Coupled with spatially-consistent grouping and region-adapted recognition, our method achieves 59.2% mIoU and 32.4% mIoU on Pascal VOC and Pascal Context benchmarks, significantly surpassing the state-of-the-art methods.

==> tables/ab_group.tex <==
\begin{table}[t]
    \centering
   \caption{\textbf{Grouping comparisons}.
   We compare two grouping ways, including STEGO and K-means algorithm with different cluster numbers.
   }
%   \vspace{1em}
   % \resizebox{1\linewidth}{!}{
   \begin{tabular}{cc|cc}
      Grouping Way &Cluster Number & mIoU & Time Cost \\
      \shline
      K-means & 2 &33.1 &1,500.0 ms \\
      K-means & 4 &47.1 & 3,000.0 ms \\    
      K-means & 6 &51.2 & 5,000.0 ms \\
      K-means & 8 &52.4 & 7,500.0 ms \\
      K-means & 10 &52.5 & 9,800.0 ms\\
      STEGO & - &54.8 &11.5 ms \\
      % \bottomrule
   \end{tabular}
  % }
    \label{tab:ab_group}
 \end{table}

==> tables/ablation.tex <==
\begin{table*}[t]
\centering
\begin{minipage}{.4\textwidth}
    \centering
   \caption{\textbf{Mask Strategies}.
   
   }
%   \vspace{1em}
   \resizebox{1\linewidth}{!}{
   \begin{tabular}{cc|cc}
      Mask Image & Patch Interaction & mIoU & Time Cost \\
      \shline
      \cmark &\xmark &39.1 &56.8 ms \\
       \xmark &\xmark &27.6 &9.3 ms\\
      \xmark &\cmark &54.8 &9.3 ms\\    
      % \bottomrule
   \end{tabular}
  }
    \label{tab:ab_mask}
\end{minipage}
\hfill
\begin{minipage}{.25\textwidth}
    \centering
   \caption{\textbf{Fine-tuning Protocols}.}
%   \vspace{1em}
   \resizebox{1\linewidth}{!}{
   \begin{tabular}{l|c}
      Fine-tuning Protocol & mIoU \\
      % \toprule
      \shline
      None &54.8 \\
      Full & 36.1 \\    
      Visual Prompt &59.2 \\
      % \bottomrule
   \end{tabular}
  }
    \label{tab:ab_finetune}
\end{minipage}
\hfill
\begin{minipage}{.32\textwidth}
    \centering
   \caption{\textbf{Assignment Mechanisms}.}
%   \vspace{1em}
   \resizebox{1\linewidth}{!}{
   \begin{tabular}{l|c}
      Assignment Mechanism & mIoU\\
      \shline
      % Baseline &54.8 \\
      Noun-to-region &59.2 \\
      Region-to-noun &52.5 \\
      Bidirectional & 56.5 \\
      % \bottomrule
   \end{tabular}
  }
    \label{tab:ab_assign}
\end{minipage}
\vspace{-1.5em}
\end{table*}

==> tables/re_ab_stage.tex <==

% \begin{table}[h]
%     \centering
%    \caption{\textbf{Ablations on stages}.
%    We retrain a STEGO with 21 types of grouped regions to match the number of Pascal VOC categories.
%    }
% %   \vspace{1em}
%    \resizebox{0.5\linewidth}{!}{
%    \begin{tabular}{cc|c}
%       1st Stage & 2nd Stage & mIoU \\
%       \shline
%       \cmark &\xmark &41.6 \\
%       \cmark &\cmark &58.9 \\    
%       % \bottomrule
%    \end{tabular}
%   }
%     \label{tab:re_ab_stage}
%  \end{table}

%  \begin{table}[h]
%     \centering
%    \caption{\textbf{Comparison with CLIPpy}.
%    }
% %   \vspace{1em}
%    \resizebox{0.5\linewidth}{!}{
%    \begin{tabular}{cc|cc}
%       Method & Pre-training & Pascal VOC & COCO \\
%       \shline
%       CLIPpy &IN1M+CC12M &50.8 &23.8 \\
%       CLIPpy &IN1M+HQITP134M &52.2 &25.5 \\
%       \midrule
%       Ours &IN1M+CC12M &55.0 & 24.9 \\    
%       Ours &IN1M+CC12M+YFCC15M &\textbf{57.3} & \textbf{25.8} \\    
%       % \bottomrule
%    \end{tabular}
%   }
%     \label{tab:re_data}
%  \end{table}

 
\begin{table}[h]
\vspace{-1.1em}
    \begin{minipage}{.15\textwidth}
       \caption{\textbf{Ablations on stages}.
       }
       \resizebox{\linewidth}{!}{
       \begin{tabular}{cc|c}
         1st Stage &2nd Stage & mIoU \\
          \shline
         \cmark &\xmark &41.6 \\
         \cmark &\cmark &58.9 \\    
          % \bottomrule
       \end{tabular}
      }
    \label{tab:re_ab_stage}
    \end{minipage}
\hfill
    \begin{minipage}{.33\textwidth}
       \caption{\textbf{Comparisons on fair datasets}.}
       \vspace{-0.7em}
       \resizebox{\linewidth}{!}{
       \begin{tabular}{cc|cc}
          Method & Pre-training & Pascal VOC & COCO \\
          \shline
          CLIPpy &IN1M+CC12M(13M) &50.8 &23.8 \\
          CLIPpy &IN1M+HQITP134M(135M) &52.2 &25.5 \\
          \midrule
          Ours &IN1M+CC12M(13M) &55.0 & 24.9 \\    
          Ours &IN1M+CC12M+YFCC15M(28M) &\textbf{57.3} &\textbf{25.8} \\    
          % \bottomrule
       \end{tabular}
      }
        \label{tab:re_data}
    \end{minipage}
\vspace{-1.65em}
\end{table}



